Bounded-Rate Multi-Mode Systems Based Motion Planning

Bounded-rate multi-mode systems are hybrid systems that can switch among a finite set of modes. Its dynamics is specified by a finite number of real-valued variables with mode-dependent rates that can vary within given bounded sets. Given an arbitrary piecewise linear trajectory, we study the problem of following the trajectory with arbitrary precision, using motion primitives given as bounded-rate multi-mode systems. We give an algorithm to solve the problem and show that the problem is co-NP complete. We further prove that the problem can be solved in polynomial time for multi-mode systems with fixed dimension. We study the problem with dwell-time requirement and show the decidability of the problem under certain positivity restriction on the rate vectors. Finally, we show that introducing structure to the multi-mode systems leads to undecidability, even when using only a single clock variable.

==> 2clocks-undec.tex <==



==> conclusion.tex <==
In this paper we studied robust reachability problem for systems modeled as
constant-rate multi-mode systems with uncertainties. 
We showed that the problem is co-NP complete in general and polynomial for
systems with fixed dimension. 
As a future work, we plan to look into robust reachability for systems with more
general dynamics and develop planning tools based on the algorithm proposed in
this paper. 


==> cut.tex <==
\subsection{Projection Along the Problem}

























Alur et al.~\cite{ATW12} presented a polynomial-time algorithm to decide if the
scheduler has a winning strategy in a reachability game on a \cmms{}.
In particular, for starting and target states in the interior of the safety set,
they characterized a necessary and sufficient condition. 
\begin{theorem} [\cite{ATW12}]
  \label{thmcms}
  The scheduler has a winning strategy in a \cmms{} $(M, n, R)$, with convex
  safety set $S$ and starting state $\px_0$ and target state $\px_t$ in the
  interior of $S$, if and only if there is  $\vec{t} \in \Rplus^{|M|}$ satisfying:
  \begin{equation}\label{eq:cmms}
    \px_0 + \sum_{i=1}^{|M|} R(i)(j) \cdot \vec{t}(i) = \px_t  \text{ for $1\leq
      j \leq n$}. 
  \end{equation}
  Notice that in such a case scheduler has a strategy to reach the target state
  precisely. 
\end{theorem}

We call  a \cmms{} \emph{reachable} if it satisfies (\ref{eq:cmms}) and we call $H$
unreachable otherwise. 
The intuition behind Theorem~\ref{thmcms} is that the scheduler has a winning
strategy if and only if it is possible to reach the target state from the
starting state in using a combination of the rate vectors. 
%% From the results of~\cite{ATW12} it also follows that whenever a winning
%% strategy exists, there is a strategy which does not look at a history or even
%% the current state, but only uses a bounded counter of size $\ell \le |M|-1$ and
%% after a history of length $k$ makes a decision only based on the number
%% $k$ modulo $\ell$. 
%% Such strategies are called \emph{periodic}.

%% It is natural to ask whether the approach of~\cite{ATW12} can be generalized 
%% to \bmms{}. 
%% Unfortunately, Example~\ref{ex22} shows that in a \bmms{} although a winning
%% strategy may exist, it may not be possible to return to the initial state, or
%% indeed visit any state twice. 
%% Another natural question to ask is whether a suitable generalization of periodic
%% strategies suffice for \bmms{}. 
%% \emph{Static} strategies are \bmms{} analog of periodic strategies that behave
%% in the same manner irrespective of the choices of the environment, i.e. for a
%% static strategy $\sigma$ we have that 
%% $\sigma(\rho) = \sigma(\rho')$ for all runs $\rho = \seq{\px_0, (m_1, 
%%   t_1), \vr_1, \px_1,  \ldots, (m_k, t_k), \vr_k, \px_k}$ and 
%% $\rho' = \seq{\px_0, (m_1, t_1), \vr'_{1}, \px_1',  \ldots, (m_k, t_k), \vr'_{k}),
%%   \px_k'}$.
%% Static strategies are often desirable in the settings where scheduler can
%% not observe the state of the system.
%% However, we observe~\cite{techreport} that except for the degenerate
%% cases when the \bmms{} contains a subset of modes which induce a safe \cmms{},
%% scheduler can never win a game on \bmms{} using static strategies. 
%% We saw an example of this phenomenon in the Introductory section as
%% Figure~\ref{geom2}.(c). 

%% This negative observations imply that to solve the schedulability games for \bmms{}
%% one needs to take a different approach. 


%% The prime~\cite{ATW12} practical motivation for studying \cmms{} was to
%% generalize results on green scheduling problem by Nghiem et al.~\cite{NBPM11}. 
%% We argue that \bmms{} are a suitable abstraction to study green scheduling problem
%% when various rates of temperature change are either uncertain or follow a complex
%% and time-varying dynamics, as shown in the following example.

%% \begin{example}[Green Scheduling]
%%   \label{example1}
%%   Consider a building with two rooms $A$ and $B$.  
%%  % Heating, ventilation, and air-conditioning (HVAC) 
%%   HVAC units in each zone can be in
%%   one of the two modes $0$ (OFF) and $1$ (ON). 
%%   We write the mode of the combined system as $m_{i,j}$ to represent 
%%   the fact that rooms $A$ and $B$ are in mode $i \in \set{0, 1}$ and $j \in
%%   \set{0,1}$, respectively. 
%%   The rate of temperature change and the energy usage for each room is given
%%   below. 
%%   \begin{center}
%%       \begin{tabular}{|p{4.5cm}|l|l|l|}
%%         \hline
%%         Zones& ON & OFF \\
%%         \hline
%%         A (temp. change rate/ usage) & -2/2& 2/1\\
%%       \hline
%%       B (temp. change/ usage) & -2/2& 2/1\\
%%       \hline
%%     \end{tabular}
%%   \end{center}
%%   Following~\cite{ATW12} we assume that the energy cost is equal to energy
%%   usage if peak energy usage at any given point in time is less than or equal to
%%   $3$ units, otherwise energy cost is $10$ times of that standard rate.
%%   It follows that to minimize energy cost the peak usage, if possible, must not
GG1










%%   be higher than $3$ units at any given time.
%%   We can model the system as a \cmms{} with modes $m_{0, 0}$, $m_{0, 1}$, and
%%   $m_{1, 0}$, because these are the only ones that have peak usage at most $3$.  
%%   The variables of the \cmms{} are the temperature of the rooms, while the
%%   safety set is the constraint that temperature of both zones should be between
%%   $65^o F$ to $75^o F$.
%%   The existence of a winning strategy in \cmms{} implies the existence of a
%%   switching schedule with energy peak demand less than or equal to $4$ units.
%%   In Figure~\ref{fig:example1}.(a) we show a graphical representation of such
%%   \cmms{} with three modes $m_{0,0}, m_{0,1}$ and $m_{1,0}$ and two variables
%%   (corresponding to the two axes).  
%%   The rate of the variables in mode $m_{0,0}$ is $(2, 2)$, in mode $m_{0,1}$ is
%%   $(2,-2)$, and in mode $m_{1,0}$ is $(-2, 2)$.
%%   \begin{figure}[t]
%%     \centering
%%     \input{geom1}
%%     \vspace{-2em}
%%     \caption{ \label{fig:example1} Restricted Multi-mode Systems}
%%     \vspace{-1em}
%%   \end{figure}

%%   Now assume that the rate of temperature change in a mode is not constant
%%   and can vary within a given margin $\varepsilon >0$.
%%   Schedulability problem for such system can best be modeled as a \bmms{} as
%%   shown in Figure~\ref{fig:example1}.(b) where the polytope of possible rate
%%   vectors is shown as a shaded region.
%%   In Figure~\ref{fig:example1}.(c) we show an \mmms{} where variables can only
%%   change with the extreme rates of the \bmms{} in  Figure~\ref{fig:example1}.(b).
%% \end{example}


==> discrete.tex <==
A strategy $\sigma$ of scheduler is called $\Delta$-sampled if for every run $r
\in \FRUNS$ if $\sigma(r) = (m, t)$ then $t$ is a multiple of $\Delta$.

\begin{theorem}
  The existence of winning strategy in a reachability game is EXPTIME-complete.
\end{theorem}
\begin{proof}
  EXPTIME-membership is straightforward as discretizing the state space using
  $\Delta$ gives an exponential size state space, and observing that solving
  reachability games are in P.
  To prove EXPTIME-hardness we show a reduction from countdown games. 
  Now we claim that the system can reach the point $(0, 0, \ldots, 0, \ldots,
  1)$ from the point $(B_1,1,0,0,\ldots,0)$ iff player 1 has a winning strategy
  in the countdown game to reach the node $n_d$ with budget $0$. 
  The intuition is that the winning strategy for player 1 in the countdown game
  directly gives a strategy for the scheduler in $\Hh$ such that a point is
  reached which has zero in the first component, and zeros everywhere else
  except for some $i$-th component. 
  Then the scheduler uses the mode $m_i$, which leads back to the initial state
  and then he can repeat the same strategy. 
  On the other hand, if player 2 has a winning strategy in the countdown game,
  this strategy can be used to get to a state from which the scheduler has no
  chance but to leave the safety set (which corresponds to not having any
  choices in the countdown game).  
  % Note on the assumption: I think the assumption ``when $(s,\ell,s')\in T$, then
  % $s\neq s'$'' is required, because when simulating a step of the countdown
  % game, we need to be always removing 1 and adding 1 at two different
  % components. The assumption with $s_1$ not being on the rhs of any rule is
  % required for the modes returning to the start to work. 
\end{proof}


==> it-is-dwell-time1.tex <==
\begin{theorem}
  The robust reachability problem with dwell-time requirement is decidable
  $\bmms{}$ where all rate vectors are positive. 
\end{theorem}
\begin{proof}
W.l.o.g assume that the starting state in $\zzero$ and the target state is
$\px_t$. 
Notice that since all the rate vectors are positive, and every mode should be
taken for at least $\Delta > 0$ time-unit, there is a bound $K$ such that the
target state is not reachable is it is not reachable in $K$ steps. 
For the robust reachability under bounded steps one can write a formula in
first-order theory of reals. 
Now the decidability of the robust reachability with dwell-time requirement for
\bmms{} with positive rate vectors follows from the decidability of the
first-order theory of reals.  
\end{proof}

\begin{theorem}
The reachability problem is $\mathsf{EXPTIME}$-hard for MMS with dwell time requirement.  
\label{thm:exphard}
\end{theorem}
\begin{proof}

We prove the result for a dwell time $\Delta \geq 1$. The result can be adapted to the case 
when $\Delta \in (0,1)$. We show the EXPTIME-hardness via a reduction from countdown games. 
A countdown game is a tuple $\mathcal{G}=(N, T, (m,B))$ where $N=\{n_1,n_2, \dots, n_k\}$ is a finite set 
of nodes, $T \subseteq N \times \mathbb{N}_{>0} \times N$ is a set of transitions, and $(m,B) \in N \times \mathbb{N}_{>0}$ 
is the initial configuration. From any configuration $(m,C)$,  player 1 chooses 
a number $l \in \mathbb{N}_{>0}$ such that there exists a transition $(m, l, m') \in T$ 
such that $l \leq C$. Among all the available transitions 
out of $m$ which are labeled $l$,   player 2 
selects an appropriate transition $(m,l,m'') \in T$. 
The new configuration is then $(m'', C-l)$. Player 1 wins when a configuration $(n,0)$ is reached, and loses 
when a configuration $(n,C)$ is reached where player 1 cannot move on, that is, 
for all outgoing transitions $(n,l,n')\in T$, we have $C-l <0$. Without loss of generality,
we assume that there are no transitions $(n,l,n) \in T$ for any $l \in \mathbb{N}_{>0}$.
Also, for any $l \in \mathbb{N}$, and any node $n$,
 let $\beta$ be the maximum number of edges 
 from $n$ with weight $l$. 
  

Given a countdown game ${\mathcal G}$, we define a BMS ${\mathcal H}$ with 
the dwell time requirement $\Delta \geq 1$ along with a bounded convex safety set, 
and a point $p$  
such that  scheduler has a strategy to reach $p$ iff player 1 
wins the countdown game. Let the initial budget of $\mathcal{G}$ be 
$\alpha$, and the initial node be $n_1$.
The constructed BMS has $k+4$ variables $\{B, n_1, \dots, n_k, z,z_1,z_2\}$. While writing 
the rate vectors of all modes, we follow the ordering $(B,n_1,n_2, \dots,n_k,z,z_1,z_2)$.
The initial mode $m_0$ of ${\mathcal H}$ has the rate vector $(\alpha, 1, 0, \dots, 0, 1,0,0)$. 
The safety set is given by $\{0 \leq n_1, \dots, n_k, z,z_1 \leq 1, 0 \leq B \leq \alpha, 0 \leq z_2 \leq \beta\}$.
The point $p$ to be reached is given by $p=(0,0,\dots,0,1,1,0)$.%%z_2 is z_3 
To reach $z=1$, exactly one unit of time has to be spent at the initial mode.  
Thus, we obtain $(\alpha, 1, 0, \dots, 0, 1,0,0)$ as the new valuation 
after spending one unit of time in the initial mode. 

For every node $n_i$ in ${\mathcal G}$ having an outgoing transition 
on some $l \in \mathbb{N}_{>0}$, we have a mode $(n_i,l)$ in the BMS 
${\mathcal H}$. The rate vector at mode $(n_i,l)$ is 
such that 
\begin{itemize}
\item $\mathcal{R}(n_i,l)(B)=-l, \mathcal{R}(n_i,l)(n_i)=-1$, 
\item $\mathcal{R}(n_i,l)(n_j)=\{0,1\}$ if 
$(n_i, l, n_j) \in T$, 
\item $\mathcal{R}(n_i,l)(n_h)=0$ for 
$(n_i, l, n_h) \notin T$. 
\item $\mathcal{R}(n_i,l)(z)=\mathcal{R}(n_i,l)(z_1)=\mathcal{R}(n_i,l)(z_2)=0$
\end{itemize}


  From the initial 
mode, scheduler has to choose one of the modes $(n_1, l)$, since going to 
any $n_j, j \neq i$ would result in the value of $n_j$ becoming negative :
spending one unit of time has resulted in the value of $n_1$ becoming 1,
the values of all other variables $n_2, \dots, n_k$ is zero. 
Thus, going to a mode $(n_j,l)$ with $j \neq 1$ would result 
 in violating the safety set, since the rate of $n_j$ is -1 at all modes $(n_j,l)$.
 The scheduler choosing a mode $(n_1,l)$ in ${\mathcal H}$ corresponds to
 the player 1 strategy of choosing a number $l$ 
at the initial node $n_1$ in ${\mathcal G}$.
While at $(n_1,l)$, the environment will pick the rate 1 for some (ideally, exactly one) 
$n_j$ that is adjacent to $n_1$, and will choose rate 0 for 
all the other $n_h$'s. This corresponds to the player 2 move 
 picking the next node in ${\mathcal G}$. 
Note that exactly one unit of time will be spent 
at $(n_1,l)$ as well, since spending more than one unit of time 
will violate the safety set. While at $(n_1,l)$, the value of 
variable $n_1$ will come back to 0, 
while the variable $n_j$ representing the next selected node $n_j$
will have value 1, and the new value of $B$ will be $\alpha-l$.
Note now that the scheduler has to select as the next mode,
one of the modes $(n_j, d)$, since these are the only places 
where the safety set will not be violated (moving to $(n_i,g), i \neq j$ will
result in the value of $n_i$ becoming negative). It can be easily seen that 
every move of the scheduler in ${\mathcal H}$ indeed corresponds 
to a move of player 1 in ${\mathcal G}$ picking a number 
at a node, while every assignment of the rate vector at a mode by the environment corresponds 
to player 2 selecting the next node in ${\mathcal G}$. 
If indeed $B$ comes down to zero while at a mode $(n_g,m)$, 
then we have $B=0,z=1$; however there will be some variable $n_d$ whose value
will be 1 ($(n_g,m,n_d) \in T$ in ${\mathcal G}$). To allow $n_d$ to come to zero, and also 
to achieve the objective $z_1=1$, we have the modes $m_{d,z_1}$, $1 \leq d \leq k$ with
\begin{itemize}
\item $\mathcal{R}(m_{d,z_1})(n_d)=-1,\mathcal{R}(m_{d,z_1})(z_1)=1$,
\item   $\mathcal{R}(m_{d,z_1})(n_h)=0, h \neq d$,
\item  $\mathcal{R}(m_{d,z_1})(B)=0$,
\item  $\mathcal{R}(m_{d,z_1})(z)=0, \mathcal{R}(m_{d,z_1})(z_2)=0$
  \end{itemize}

Note that exactly one unit has to be spent at the chosen mode $m_{d,z_1}$; moreover,
if the scheduler comes to any mode $m_{d,z_1}$ when $B > 0$, the reachability objective cannot be realised.  

Consider now, at a mode $(n_i,l)$,  the environment strategy of assigning rate 0 
to all $n_j$ that are adjacent to $n_i$ in ${\mathcal G}$.
In this case, scheduler cannot move to any of the modes $(n_j,d)$ for 
$1 \leq j \leq k$, since this will violate the safety set. Note that the modes 
$m_{d,z_1}$, $1 \leq d \leq k$ will not help the scheduler either.
To offset this environment strategy, 
we create {\it zero correction} modes $c_0, c_1, \dots, c_{\alpha}$ such that
for $0 \leq j \leq \alpha$,
\begin{itemize}
\item $\mathcal{R}(c_j)(B)=-j,\mathcal{R}(c_j)(z_1)=1$
 \item $\mathcal{R}(c_j)(n_i)=0, 1 \leq i \leq k$,
 \item $\mathcal{R}(c_j)(z)=\mathcal{R}(c_j)(z_2)=0$.
\end{itemize}
If the environment makes the mistake of not choosing any next node, 
the scheduler can win by moving to the appropriate zero correction mode, choosing the 
right rate for $B$ (the remaining quantity needed to achieve 0), and achieve the reachability objective, 
by spending one unit of time in the chosen mode $c_j$.


Another possible strategy of the environment, while at a mode
$(n_i,l)$, is to assign rate 1 to more than one  
 $n_j$ that is adjacent to $n_i$ in ${\mathcal G}$. In this case, 
 the zero correction modes $c_j$ alone, or along with modes 
 $m_{d,z_1}$ do not help, since $z_1$ can only grow to 1.
Thus, it is not possible to use these two types of modes together. 
 To rectify this mistake, we create 
the  {\it non-zero correction} modes
$m_1, m_2, \dots, m_k$ and the $(\beta-1)(\alpha+1)$ modes $M_{i,j}$ 
$0 \leq i \leq \alpha, 2 \leq j \leq \beta$ such that

\begin{itemize}
\item $\mathcal{R}(m_i)(n_i)=-1,\mathcal{R}(m_i)(z_2)=1$, 
\item $\mathcal{R}(m_i)(n_j)=0, j \neq i, 
\mathcal{R}(m_i)(B)=0,$
\item $\mathcal{R}(m_i)(z)=0=\mathcal{R}(m_i)(z_1)$,
\item $\mathcal{R}(M_{i,j})(B)=-i,\mathcal{R}(M_{i,j})(z_2)=-j$,
\item $\mathcal{R}(M_{i,j})(z_1)=1$,
\item $\mathcal{R}(M_{i,j})(n_h)=0, 1 \leq h \leq k$.  
\end{itemize} 
If more than one $n_j$ (say $h \geq 2$) is assigned rate 1 by the environment at some $n_i$, 
the scheduler can visit the $h$ appropriate modes $m_j$, obtaining 
the values of those $h$ variables $n_j$ to zero and $z_2=h \geq 2$. 
Note that visiting modes $m_1, \dots, m_k$, the variable $z_2$ can grow to atmost $\beta$, the maximum outdegree 
corresponding to any node $n_i$ and label $l \in \mathbb{N}$. 

This is followed by choosing an appropriate mode $M_{i,h}$ where scheduler 
can obtain $z_2=0, z_1=1$ and $B=0$. Note that if the environment had assigned a rate 1 to a 
unique variable $n_j$ (hence, picked a unique successor node), then 
the value of $z_2$ will be 1 on visiting $m_j$. Scheduler cannot go to more than one $m_j$ in that case, since it will result in some variable $n_h$ violate the safety requirement. If $z_2 \leq 1$, then visiting 
any of the modes $M_{i,j}$ will not help either, since the rate of $z_2$ is $-j$ in $M_{i,j}$, 
for $j \geq 2$.


To summarize, scheduler has a winning strategy in ${\mathcal H}$ iff player 1 has a winning strategy 
in ${\mathcal G}$. The environment strategy is to assign at each at each mode $(n_i,l)$, 
rate 1 to a unique variable $n_j$, among the adjacent nodes $n_j$ to $n_i$. Under this, 
the scheduler can win in ${\mathcal H}$ iff he wins in ${\mathcal G}$. Whenever 
the environment makes an error by assigning rate 1 to none, or more than one 
 variable $n_j$ in any mode $(n_i,l)$, the scheduler has a winning strategy in 
 ${\mathcal H}$.
 \end{proof}




==> krishna-ctl-sha.tex <==
We also observe that CTL model checking for weak singular hybrid automata is
already hard for \PSPACE{} by using a reduction from subset sum games~\cite{FJ13}.
\begin{theorem}
   \label{thm:ctl-weak-sha}
   CTL model checking of weak SHAs with two clock variables is \PSPACE{}-hard. 
 \end{theorem}
We conjecture that the problem can be solved in \PSPACE{}, however decidability
of the problem is currently open. 





==> wsha-clocks.tex <==
\input{merged-fig-undec}
In this section, we present two variants  of WSHA and show that both lead to
undecidability of the reachability problem. 
The first  variant that we consider is weak singular hybrid automata
extended with discrete updates on the variables even inside the strongly
connected components. 

\begin{theorem}
  \label{thm:sha-undec-three-var}
  The reachability problem is undecidable for three variable WSHAs with discrete
  updates. 
 \end{theorem}
\begin{proof}
  We show a reduction from the halting problem for two-counter Minsky machines
  ${\cal M}$. 
  The variables $x,y,z$ of the SHA  have global invariants $0 \leq x \leq 1$, $0
  \leq y,z\leq 5$ respectively. 
  The counters $c_1, c_2$ of two-counter machine are encoded in variables $y$ and
  $z$ as 
  \[
  y=5-\frac{1}{2^{c_1}} \text{ and  } z=5-\frac{1}{2^{c_2}}.
 \]
  To begin, we have $c_1=c_2=0$, hence $y=z=4$, and $x=0$.
  The rates of $x,y,z$ are indicated by 3-tuples inside the modes of the SHA. 
  Likewise, the discrete updates on $x,y,z$ are also indicated by a 3-tuple 
  on the transitions.  We construct widgets for each of the increment/decrement and zero check instructions. 
  Each widget begins with $x=0,y=5-\frac{1}{2^{c_1}}$ and $z=5-\frac{1}{2^{c_2}}$, where $c_1,c_2$ are the current 
  values of the counters. 
  \begin{itemize}
  \item {\bf (Increment and Decrement Instructions).}
    Let us first consider increment instruction 
    \[
    l : c_1 := c_1 + 1 \text{ goto } l'.
    \] 
    The left side widget of Figure~\ref{z-c1} depicts the increment widget. 
    This widget starts with a mode labeled $l$, and  ends in a mode labeled $l'$. 
    
    On entering $l$, we have $x=0$ and $y=5-\frac{1}{2^{c_1}}$. A time of $k=\frac{1}{6}[5-\frac{1}{2^{c_1}}]$ has 
    to be spent at $l$, giving $x=\frac{1}{6}[5-\frac{1}{2^{c_1}}]$ and $y=0$. If a time $>k$ is spent at $l$, then 
    we obtain $y=5-\frac{1}{2^{c_1}}-6[k+\eta] <0$, violating the invariants of $y$. Likewise, if a time $<k$ is spent at $l$, 
    then we obatin $y=5-\frac{1}{2^{c_1}}-6[k-\eta]=6\eta$, which would make $y=5+6 \eta > 5$ on taking the transition from 
    $l$ to $A$. Thus, on entering $A$, we have $y=5$ and $x=k$. At $A$, a time $k_1=\frac{1}{6}$ is spent, obtaining 
    $x=k+k_1=1-\frac{1}{6.2^{c_1}}$, and $y=0$. If a time $<k_1$ is spent at $A$, we get $y=5-30(k_1-\kappa)=30 \kappa$
    which would violate the invariants  of $y$ on taking the transition from $A$ to $B$. Similarly, 
    if a time $>k_1$ was spent at $A$, we get $y=5-30(k_1+\kappa)<0$ again violating the invariants of $y$. 
    Thus, on reaching $B$, we have $x=1-\frac{1}{6.2^{c_1}}$ and $y=5$. To reach $l'$, we spend 
    $\frac{1}{6.2^{c_1}}$ time at $B$, and get $x=0$, and $y=5-3(\frac{1}{6.2^{c_1}})=5-\frac{1}{2^{c_1+1}}$. 
    Note that if a time less than $\frac{1}{6.2^{c_1}}$ is spent at $B$, then $x$ would violate 
    its invariants while taking the transition to $l'$.  Likewise, 
    if a time $>\frac{1}{6.2^{c_1}}$ is spent at $B$, $x$ would violate its
    invariants.
    
    This widget can be modified to simulate the instructions increment counter $c_2$,
    decrement counters $c_1$ and decrement counter $c_2$,respectively,  by changing  the cost rate of $z$ at
    $B$ to -3, the cost rate of $y$ at $B$ to -12, and the cost rate of $z$ at $B$
    to $-12$, respectively.  
    
  \item {\bf (Zero Check Instruction).}
    We next consider the zero check instruction:
    \[
    l: \text{ if } c_1=0 \text{ goto } l' \text{ else  goto } l''.
    \]
 The right side widget of Figure~\ref{z-c1} depicts the zero check widget. 
 The zero check widget  starts in a mode $l$ and reaches either the mode $l'$ or mode $l''$.
 
 Assume that $c_1=0$. Then $y=4$. Then the only possible transition to take is the one from $l$ to $A$, which 
makes $y=5$. Note that no time is spent at $l$ in this case, since it would violate 
the invariants of $y$ while moving to $A$. Thus, at $A$ we have $y=5,x=0$. No time is spent at $A$ since 
it would make $x <0$. On reaching $l'$, we therefore have $y=4$. Note that if $c_1=0$, then we cannot take the transition 
from $l$ to $B$ since it cannot meet invariants $y \leq 5$
and $x \leq 1$ simultaneously : Unless one time unit is spent at $l$, $y$ would violate its invariants 
on taking the edge to $B$. In this case, $x$ will become 2, violating $0 \leq x \leq 1$. 


If $y=5-\frac{1}{2^{c_1}}$ with $c_1 >0$, then we take the transition from $l$ to $B$ after spending some time 
at $l$. We cannot take the transition from $l$ to $A$, since that would violate 
the invariants of $y$. Thus, we go to $B$ when $c_1 >0$. The time spent at $l$ is some $0<\eta < 1$. 
This gives $y=5-\frac{1}{2^{c_1}}+\eta$ and $x=2\eta$. 
If $\eta > \frac{1}{2^{c_1}}$, then the invariants of $y$ get violated. If $\eta < \frac{1}{2^{c_1}}$, then 
on taking the transition to $B$, we obtain $y=5-\frac{1}{2^{c_1}}+\eta-5<0$, again violating 
the invariants of $y$. 
Hence, $\eta=\frac{1}{2^{c_1}}$, and we reach $B$ with $x=2\eta,y=0$.
Now at $B$, a time $1-2\eta$ is spent, reaching $C$ with $x=0, y=\frac{1}{2}-\eta$. 
If a time $< 1-2\eta$ is spent at $B$, then $x$ will violate its invariants 
on taking the transition to $C$; if a time $>1-2\eta$ is spent at $B$, $x$ will exceed 1.
At $C$, we thus have $x=0$ and $y=\frac{1}{2}-\frac{1}{2^{c_1}}$. 
At $C$, $\frac{1}{2}$ units of time is spent, obtaining $x=1$ and $y=1-\frac{1}{2^{c_1}}$, 
so that on reaching $D$, $x=0$ and $y=1-\frac{1}{2^{c_1}}$. Finally, $l''$ is reached with 
$x=0$ and $y=5-\frac{1}{2^{c_1}}$. 
\end{itemize}
It is straightforward to see that the modules for increment, decrement, and zero
check simulate the two counter machine. There is a mode HALT corresponding to the HALT  instruction. 
The halting problem for two counter machines is thus  reduced to the
reachability of the mode HALT. 
\end{proof}

We also show that extending even constant-rate multi-mode systems with one unrestricted
clock variable lead to undecidability.  
% 
 \begin{theorem}
   \label{thm:sha-undec-three-var-one-clock}
 The reachability problem is undecidable for CMS with three variables and one
unrestricted clock. 
 \end{theorem}

 
 

==> wsha.tex <==
Constant-rate multi-mode systems, introduced by Alur et al.~\cite{ATW12}, are
hybrid systems that can switch freely among a finite set of modes, and whose
dynamics is specified by a finite number of real-valued variables with
mode-dependent constant rates.  
They showed that the natural reachability and schedulability problem for such
systems can be decided in polynomial time. 
Our main motivation in studying weak singular hybrid automata is to generalize
constant-rate multi-mode systems further while still preserving the decidability
of these key problems, and to study model-checking problem for the
generalization of multi-mode systems.
We begin this section by formally introducing constant-rate multi-mode systems
and review the decidability of reachability and schedulability problems for this
class. 
We later present the weak singular hybrid automata model and show the decidability
of various verification problems. 

\subsection{Constant-Rate Multi-Mode Systems}
\begin{definition}[Constant-Rate Multi-Mode Systems]
  An SHA $\Hh = (M, M_0, \Sigma, X, \Delta, I, F)$ is a \emph{constant-rate
    multi-mode system} (CMS) if 
  \begin{itemize}
  \item 
    there is a bounded and open polytope  $S$, called the safety set, such that for
    all modes $m \in M$ we have that $I(m) = S$, and
  \item 
    all the modes in  $M$ form a strongly-connected-component, and for every
    mode $m, m' \in M$ if there is a transition $(m, G, a, R, m') \in \Delta$
    then $G=\top$, and $R=\emptyset$. 
  \end{itemize}
\end{definition}
We have slightly modified the definition of the CMS to adapt it to the
presentation used in this paper.
Moreover, we have restricted the safety set to be an open set to avoid problems
in reaching a valuation using infinitely many transitions. 

Notice that there is no structure in a CMS in the sense that all of the modes
can be chosen in arbitrary order as long as the safety set is not violated. 
Alur et al.~\cite{ATW12} showed that due to lack of structure, the
schedulability and the reachability problems for CMS can be reduced to LP
feasibility problem, and hence can be solved in polynomial time. 
\begin{theorem}[Reachability Problem~\cite{ATW12}]
  \label{thm:mms-reach}
  Given a CMS $\Hh$, a starting valuation $\nu$ and a target polytope $\Tt$
  such that both $\nu$ and $\Tt$ are in the safety set of $\Hh$, the
  reachability problem $\Reach(\Hh, \nu, \Tt)$ can be decided in polynomial time. 
\end{theorem}
\begin{proof}[(Sketch)]
  Let $\Hh = (M, M_0, X, \Delta, I, F)$ be a CMS with the safety set $S$ and 
  the target  polytope $\Tt$ be given as a system of linear inequalities $AX
  \leq \vb$. 
  Moreover assume that $\nu$ and $\Tt$ are in the safety set $S$.
  Alur et al. showed that the target set $\Tt$ is reachable from the valuation
  $\nu$ if and only if the following linear program is feasible: 
  \begin{eqnarray}
    \nu + \sum_{m \in M} F(m) \cdot t_m &=& \nu' \nonumber\\
    A \nu' &=& \vb \label{eqnreachmms}\\
    t_m & >= & 0 \text{ for all $m \in M$}.\nonumber
  \end{eqnarray}
  If this linear program is not feasible, then it is immediate that it is not
  possible to reach any valuation in $\Tt$  from $\nu$ using modes in any
  sequence from $\Hh$. 
  On the other hand, if the program is feasible, and as long as both the
  starting valuation and the target set are strictly inside the safety set, a
  satisfying assignment $\seq{t_m}_{m \in M}$ can be used to make progress
  towards $\Tt$ by scaling $t_m$'s appropriately without leaving the safety
  set. 
  Since the feasibility of the linear program can be decided in polynomial time,
  it follows that reachability for the CMS can be decided in polynomial time. 
\end{proof}

\begin{theorem}[Schedulability Problem~\cite{ATW12}]
\label{thm:mms-sched}
Given a CMS $\Hh$ and a starting valuation $\nu$, the schedulability problem 
  $\Sched(\Hh, \nu)$ can be decided in polynomial time. 
\end{theorem}
\begin{proof}[(Sketch)]
  Let $\Hh = (M, M_0, X, \Delta, I, F)$ be a CMS with the safety set $S$, and
  initial valuation $\nu$.  
  In this case, Alur et al. showed that there exists a non-Zeno run from
  arbitrary valuation in the safety set  if and only if the following linear
  program is feasible:   
  \begin{eqnarray}
    \sum_{m \in M} F(m) \cdot t_m &=& \vzero \nonumber\\
    \sum_{m \in M} t_m  &=& 1  \label{eqnschedmms}\\
    t_m & >= & 0 \text{ for all $m \in M$}.\nonumber
  \end{eqnarray}
  If this linear program is not feasible, then by Farkas's lemma it follows that
  there is a vector $\vv$ such that taking any mode for nonnegative time makes
  some progress in the direction of $\vv$. 
  Hence any non-Zeno run will eventually leave the safety set. 
  On the other hand, if the program is feasible, then a 
  satisfying assignment $\seq{t_m}_{m \in M}$ can be scaled down to stay in a
  ball of arbitrary size around the initial valuation. 
  Hence, if the starting valuation is strictly in the interior of the safety
  set, the feasibility of the linear program~(\ref{eqnschedmms}) imply the
  existence of a non-Zeno run. 
\end{proof}

\subsection{Syntax and Semantics}
\emph{Weak singular hybrid automata} can be considered as generalized
constant-rate multi-mode systems with structure, and thus bringing the CMS
closer to singular hybrid automata.  
The restriction on weak singular hybrid automata (WSHA) ensures that the
strongly connected components of WSHA form  CMS, and thus recovering the
decidability for the reachability and the schedulability problem.  
Formally we define weak singular hybrid automata in the following manner. 

\begin{definition}[Weak Singular Hybrid Automata]
  A weak singular hybrid automaton $\Hh = (M, M_0, \Sigma, X, \Delta, I, F)$ is
  a SHA with the restriction 
  that there is a partition on the set of modes $M$ characterized by a function
  $\varrho: M \rightarrow \Nat$ assigning \emph{ranks} to the modes such that
  \begin{itemize}
  \item  
    for every transition $(m, G, a, R, m') \in \Delta$ we have that    
    $\varrho(m) \leq \varrho(m')$, and 
  \item  
    for every rank $i$ the set of modes $M_i = \set{m \::\: \varrho(m) = i}$ is
    such that 
    \begin{itemize}
    \item 
      there is a bounded and open polytope $S_i$, called the safety set of $M_i$,
      such that  for all modes $m \in M_i$ we have that $I(m) = S_i$; and
    \item
      all the modes in $M_i$ form a strongly-connected-component, and for every
      mode $m, m' \in M_i$ if there is a transition $(m, G, a, R, m') \in \Delta$
      then $G=\top$, and $R=\emptyset$. 
    \end{itemize}
  \end{itemize}
Observe that every CMS is a weak singular hybrid automaton (WSHA), and every
strongly connected component of a WSHA is a CMS. 
\end{definition}

Observe that for every (finite or infinite) run 
\[
  r = \seq{(m_0, \nu_0), (t_1, a_1), (m_1, \nu_1), \ldots}
\]
of a WSHA we have
that $\varrho(m_i) \leq \varrho(m_j)$ for every $i \leq j$.
We define the type $\Gamma(r)$ of a finite run 
\[
r = \seq{(m_0, \nu_0), (t_1, a_1), (m_1, \nu_1), \ldots, (m_k, \nu_k)}
\]
as a finite sequence of ranks (natural numbers) and actions  
$\seq{n_0, b_1,  n_1,\ldots, b_p, n_p}$ defined inductively in the following manner: 
\begin{eqnarray*}
  \Gamma(r) = 
\begin{cases}
  \seq{\varrho(m_0)} & \text{ if $r = \seq{(m_0, \nu_0)}$}\\
  \Gamma(r') \oplus (a, \varrho(m)) & \text{ if $r = r'::\seq{(t, a), (m, \nu)}$},
\end{cases}
\end{eqnarray*}  
where $::$ is the cons operator that appends two sequences, while 
for a sequence $\sigma = \seq{n_0, b_1, n_1, \ldots, b_p, n_p}$, $a \in \Sigma$, and $n \in
\Nat$ we define $\sigma \oplus (a, n)$ to be equal to $\sigma$ if $n_p = n$ and
$\seq{n_0, b_1, n_1, \ldots, n_p, a, n}$ otherwise.
Intuitively, the type of a finite run gives the (non-duplicate) sequence of
ranks of modes and actions appearing in the run, where action is stored only
when a transition to a mode of higher rank happens. 
We need to remember only these actions since transitions that stay in the modes
of same rank do not reset the variables. 

Since there are only finitely many ranks for a given WSHA, it follows that for
every infinite run 
\[
r = \seq{(m_0, \nu_0), (t_1, a_1), (m_1, \nu_1), \ldots}
\] there
exists an index $i$ such that  for all $j \geq i$ we have that $\varrho(m_i) =
\varrho(m_j)$. 
With this intuition we define the type of an infinite run $r$ as the type of the
finite prefix of $r$ till index $i$.
Let $\Gamma_\Hh$ be the set of run types of a WSHA $\Hh$.

\subsection{Reachability Problem}
Given a run type $\sigma = \seq{n_0, b_1, n_1, \ldots, b_p, n_p}$ an initial
valuation $\nu_0$ and a bounded and convex target polytope $\Tt$ given as $A X
\leq \vb$,we say that $\sigma$ leads the WSHA $\Hh$ from $\nu$ to $\Tt$ if the
following linear program is feasible: 
for every $ 0 \leq i \leq p$ and  $m \in M_{n_i}$ there are 
$\nu_{n_i}, \nu_{n_i}' \in \Real^{|X|}$ and  $t_i^m \in \Rplus$ such that    
\begin{eqnarray}
  \nu_0 &=& \nu_{n_0} \nonumber \\
  \nu_{n_p}' & \in & \Tt \nonumber\\
  \nu_{n_i}, \nu_{n_i}'  & \in & S_{M_{n_i}} \text{ for all $0 \leq i \leq p$} 
  \nonumber \\
  \nu_{n_i}   & \in & G(b_i) \text{ for all $0 < i \leq p$}
  \nonumber \\
  \nu_{n_{i+1}}(j) &=& 0 \text{ for all $x_j \in R(b_{i+1})$ and  $0 < i \leq p$}
  \nonumber \\
   \nu_{n_{i+1}}(j) &=& \nu_{n_i}'(j)  \text{ for all $x_j \not \in R(b_{i+1})$ and  $0 < i \leq p$}
  \nonumber \\
   \nu_{n_i}'  & = & \nu_{n_i} + \sum_{m \in M_{n_i}} F(m) \cdot t_i^m \text{
     for all $0 \leq i \leq p$}\nonumber\\% \label{eqn-wsha-reach}\\
  t_i^m  &\geq&  0 \text{ for all $0 \leq i \leq p$ and  $m \in M_{n_i}$} \nonumber
\end{eqnarray}
These constraints check whether it is possible to reach some valuation in the
target polytope while satisfying the guard and constraints of the WSHA, while
exploiting the fact that modes of same rank can be applied an arbitrary number
of time in an arbitrary order. 

The proof of the following proposition follows the same structure as the proof
of Theorem~\ref{thm:mms-reach}, and hence we omit the proof. 
\begin{proposition}
  \label{prop:type-and-run}
  Let $\Hh$ be a WSHA, $\nu$ be a valuation, and $\Tt$ be a target convex
  polytope. 
  There exists a run type $\sigma$ of $\Hh$ that leads $\Hh$ from $\nu$ to $\Tt$
  if and only if there exists a run of $\Hh$ from $\nu$ to $\Tt$.  
\end{proposition}
% 
\begin{theorem}
  \label{thm:wsha-reach-np-hard}
  The reachability problem for weak singular hybrid automata  is NP-complete.
\end{theorem}
\begin{proof}
  From Proposition~\ref{prop:type-and-run} it follows that to decide the
  reachability problem for WSHA it is sufficient to check that there exists a
  run type that leads the WHSA from initial valuation to the target polytope. 
  Since total number of run types are exponential in the size of WSHA, and
  checking whether a run type leads from $\nu$ to $\Tt$ can be performed in
  polynomial time, the reachability of WSHA is in NP.

  To show NP-hardness we reduce the \emph{subset-sum problem}, which is known to
  be \NPC{}, to solving the reachability problem in a WSHA.
  Given a set $A = \{a_1, a_2\cdots a_n\}$  of $n$ integers and another integer $k$,
  the subset-sum problem asks to whether there exists a non-empty set $T
  \subseteq A$ that sums to $k$. 
  
  Given the set $A$ and the integer $k$, we construct a WSHA $\Hh$ with $n+3$
  variables $x_0,x_1, \dots, x_{n+2}$, $2n+1$ modes $m_0, \dots, m_{2n}$ and
  $2n$ transitions, such that a particular target polytope $\Tt$ is reachable in
  the WSHA iff there is a non-empty subset $T \subseteq A$ that sums up to $k$.

The rates in the modes $m_i (0\leq i\leq 2n)$ are given as follows ($r_i$ represents
$(F(m_i))$:
\begin{itemize}
\item[$\bullet$] $\vr_0(x_0) =1, \vr_0(x_{n+1}) = \vr_0(x_{n+2}) = 0$, and
$\vr_0(x_i) = a_i$, where $1\leq i\leq n$
\item[$\bullet$] $\vr_{2j-1}(x_j) = -a_j$, $\vr_{2j-1}(x_{n+1}) = a_j$,
$\vr_{2j-1}(x_{n+2}) = 1$, and $\vr_{2j-1}(x_0)$ = $\vr_{2j-1}(x_i) = 0$,
where $1\leq i\neq j\leq n$
\item[$\bullet$] $\vr_{2j}(x_j) = -a_j$, and $\vr_{2j}(x_0) = \vr_{2j}(x_i) =$
$\vr_{2j}(x_{n+1}) = \vr_{2j}(x_{n+2}) = 0$,
 where $1\leq i\neq j\leq n$
\end{itemize}
The transitions in the WSHA are as follows:
\begin{itemize}
\item[$\bullet$] There are edges from $m_0$ to $m_1$ and to $m_2$.
\item[$\bullet$] There are edges from $m_{2j-1}$ and from $m_2j$ to $m_{2j+1}$ and to $m_{2j+2}$, $1\leq j\leq n-1$
\end{itemize}
We now claim that the polytope $\Tt$, given by the set of points $\px$
such that $\px(0) = 1$, $\px(i) = 0$, $1\leq i\leq n$, $\px(n+1) = k$
and $\px(n+2) \in [1,n]$, is reachable from the point $\vzero$
iff there is a subset $T$ of $A$ that sums up to $k$.

We first prove that if there is a non-empty $T$ that sums to $k$, then $\Tt$
is reachable from $\vzero$.
It is evident that the point $(1,0,0\cdots,k,|T|) \in \Tt$ can be reached
by taking the following sequence of (time, mode) having length $n+1$:
\[
\seq{(1,m_0), (1, l_1), (1, l_2)\cdots, (1, l_n)}
\]
where $l_i = m_{2i-1}$ if $a_i \in T$, otherwise $l_i = m_{2i}$.

We now prove that if the WSHA $\Hh$ reaches a point in $\Tt$ starting from $\vzero$,
then there is a non-empty subset of $A$ that sums to $k$.
For this, note that since $m_{2j-1}$ or $m_{2j}$ ($1\leq j\leq n$) cannot be
reached from one another in the underlying graph, atmost one of them can
occur in any path in the WSHA.
Also, since $\pt(0) = 1$, $\forall \pt \in \Tt$, and since for all modes $m$ apart from
$m_0$, $F(m)(x_0) = 0$, the mode $m_0$ must be taken for exactly unit time.
This means that the first step in any run that reaches $\Tt$ is $(t_0 = 1, m_0)$.
Now, after the first step, the WSHA reaches the valuation $(1, a_1, a_2\cdots a_n,0,0)$.
In order to reach $\Tt$, all the coordinates $x_1$ to $x_n$ must go to zero.
However, since the rate of $a_i$ is non-zero only in the modes $m_{2i-1}$ and $m_{2i}$, and
because atmost one of $m_{2i-1}$ and $m_{2i}$ can be taken, we conclude that exactly one
of $m_{2i-1}$ and $m_{2i}$ is taken for a 1 unit of time.
(For the sake of simplicity, we can assume wlog that each of $a_i\neq 0$). 
 Hence, any reachable run will comprise of $n+1$ steps.
Also, since we demand that $\pt(n+2) \in [1,n]$ and the rate of $x_{n+2}$ is non-zero
only in the modes $m_{2i-1}$ ($1\leq i\leq n$), atleast one of the modes $m_{2i-1}$
is necessarily taken. 
Now consider the run that reaches $\Tt$:
\[
\seq{(1, m_0), (1, l_1), (1, l_2)\cdots, (1, l_n)}
\]
It is clear that the set $\{a_i | l_i = m_{2i-1}\}$ is a non-empty subset that sums to $k$.
Figure \ref{nphard} gives an illustration of the WSHA construction for a set $\{1,2,-3\}$. 
\end{proof}
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.8cm,
  semithick]
  \tikzstyle{every state}=[fill=black!30!white,minimum size=3em,rounded rectangle]
 \node[state] at (1.7,1.5) (A0) {$\begin{array}{c}m_0 \\ (1,1,2,-3,0,0) \end{array}$} ;
 \node[state] at (0,0) (A1) {$\begin{array}{c}m_1 \\ (0,-1,0,0,1,1) \end{array}$} ;
 \node[state] at (0,-2) (B1) {$\begin{array}{c}m_3 \\ (0,0,-2,0,2,1) \end{array}$} ;
 \node[state] at (0,-4) (B2) {$\begin{array}{c}m_5 \\ (0,0,0,3,-3,
 1) \end{array}$} ;
   \node[state] at (4,0) (A) {$\begin{array}{c} m_2 \\ (0,-1,0,0,0,0) \end{array}$} ;
   \node[state] at (4,-2) (B) {$\begin{array}{c} m_4 \\ (0,0,-2,0,0,0) \end{array}$} ;
   \node[state] at (4,-4) (C) {$\begin{array}{c} m_6 \\ (0,0,0,3,0,0) \end{array}$} ;
   
      \path (A0) edge node [above]{} 
                    (A);
                    \path (A0) edge node [above]{} 
                    (A1);
      \path (A1) edge node [above]{} 
                    (B);
                    \path (A1) edge node [above]{} 
                    (B1);
     \path (A) edge node [above]{} 
                    (B);
                    \path (A) edge node [above]{} 
                    (B1);
     \path (B1) edge node [above]{} 
                    (B2);
                    \path (B1) edge node [above]{} 
                    (C);
\path (B) edge node [above]{} 
                    (B2);
       \path (B) edge node [above]{} 
                    (C);
 \end{tikzpicture}
\caption{Constructed WSHA for a set $\{1,2,-3\}$}
\label{nphard}
\end{center}
\end{figure}

\subsection{Schedulability Problem}
Given a run type $\sigma = \seq{n_0, b_1, n_1, \ldots, b_p, n_p}$ and an initial
valuation $\nu_0$, we say that $\sigma$ schedules the WSHA $\Hh$ from $\nu$ to $\Tt$ if the
following linear program is feasible: 
for every $ 0 \leq i \leq p$ and  $m \in M_{n_i}$ there are $\nu_{n_i},
\nu_{n_i}' \in \Real^{|X|}$ and  $t_i^m \in \Rplus$ such that     
\begin{eqnarray}
  \nu_0 &=& \nu_{n_0} \nonumber \\
  \nu_{n_i}, \nu_{n_i}'  & \in & S_{M_{n_i}} \text{ for all $0 \leq i \leq p$}
  \nonumber \\
  \nu_{n_i}   & \in & G(b_i) \text{ for all $0 < i \leq p$}
  \nonumber \\
  \nu_{n_{i+1}}(j) &=& 0  \text{ for all $x_j \in R(b_{i+1})$ and  $0 < i \leq p$}
  \nonumber \\
  \nu_{n_{i+1}}(j) &=& \nu_{n_i}'(j)  \text{ for all $x_j \not \in R(b_{i+1})$ and  $0 < i \leq p$}
  \nonumber \\
  \nu_{n_i}'  & = & \nu_{n_i} + \sum_{m \in M_{n_i}} F(m) \cdot t_i^m \text{
    for all $0 \leq i \leq p$} \nonumber\\%\label{eqn:wsha-sched}\\
  t_i^m  &\geq&  0 \text{ for all $0 \leq i \leq p$ and $m \in M_{n_i}$} \nonumber\\ 
  \vzero &=& \sum_{m \in M_{n_p}} F(m) \cdot t_p^m  \nonumber\\
  1 &=& \sum_{m \in M_{n_p}} t_p^m \nonumber
\end{eqnarray}
These constraints check whether it is possible to reach some mode with the
highest rank while satisfying the guard and constraints of the WSHA, and
schedule the system forever in the CMS defined by the SCCs of the highest rank in
the type. 

The proof of the following proposition follows from the proof
of Theorem~\ref{thm:mms-sched} and Proposition~\ref{prop:type-and-run}, and
hence omitted. 
\begin{proposition}
  \label{prop:type-and-sched}
  Let $\Hh$ be a WSHA and $\nu$ be a valuation.
  There exists a run type $\sigma$ of $\Hh$ that schedules $\Hh$ from $\nu$ 
  if and only if there exists a non-Zeno infinite run of $\Hh$ from $\nu$. 
\end{proposition}

\begin{theorem}
  The schedulability problem for WSHA is NP-complete. 
\end{theorem}
\begin{proof}
  From Proposition~\ref{prop:type-and-sched} it follows that to decide the
  schedulability problem for WSHA it is sufficient to check that there exists a
  run type that schedules the WHSA from the initial valuation.
  Since total number of run types are exponential in the size of WSHA, and
  checking whether a run type schedules from $\nu$ can be performed in
  polynomial time (LP feasibility), the schedules in WSHA can be decided in
  polynomial time.  
  The NP-hardness of the result follows from a similar reduction from subset sum
  problem as shown in Theorem~\ref{thm:wsha-reach-np-hard}. 
\end{proof}

% \input{wsha-reach}
%\subsection{Schedulability Problem}
%\input{wsha-sched}

\subsection{LTL Model Checking}
\begin{theorem}
  The LTL model-checking problem for WSHA is PSPACE-complete.
\end{theorem}
\begin{proof}
  Let $(\Hh, \Pp, L)$ be a weak Kripke SHA and let $\phi$ be an LTL property. 
  From the standard LTL to B\"uchi automata construction~\cite{VW86} the negation
  of $\phi$ can be converted to B\"uchi automata $\Aa_{\neg \phi}$  whose size
  is exponential in the size of $\phi$.
  The LTL model checking problem then reduces to solving a schedulability
  problem for the product of original automaton and $\Aa_{\neg \phi}$. 
  We observe that the product of a weak SHA $\Hh$ and $\Aa_{\neg \phi}$ remains
  weak SHA, since variables occur only in the WSHA.  
  The LTL model checking problem thus reduces to the schedulability problem for
  a weak SHA of size exponential in the size of original problem, and hence can
  be decided using standard polynomial space algorithm.
  PSPACE-hardness of the problem follows as the LTL model checking over finite
  automata is already PSPACE-complete. 
\end{proof}

% \input{wsha-ltl}

\subsection{CTL Model Checking}
\input{krishna-ctl-sha} 


